NTIRE 2025 Challenge on UGC Video Enhancement: Methods and Results

This paper presents an overview of the NTIRE 2025 Challenge on UGC Video Enhancement. The challenge constructed a set of 150 user-generated content videos without reference ground truth, which suffer from real-world degradations such as noise, blur, faded colors, compression artifacts, etc. The goal of the participants was to develop an algorithm capable of improving the visual quality of such videos. Given the widespread use of UGC on short-form video platforms, this task holds substantial practical importance. The evaluation was based on subjective quality assessment in crowdsourcing, obtaining votes from over 8000 assessors. The challenge attracted more than 25 teams submitting solutions, 7 of which passed the final phase with source code verification. The outcomes may provide insights into the state-of-the-art in UGC video enhancement and highlight emerging trends and effective strategies in this evolving research area. All data, including the processed videos and subjective comparison votes and scores, is made publicly available at https://github.com/msu-video-group/NTIRE25_UGC_Video_Enhancement.

==> figures/Nobody_description/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> figures/Nobody_description/sections/results.tex <==
\section{Results}

\input{sections/solutions.tex}

==> figures/Nobody_description/sections/solutions.tex <==

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\columnwidth]{NTIRE 2025 UGC Video Enhancement Description Template/figures/results.png}
    \caption{Our video enhancement results.}
    \label{fig:results}
\end{figure}

\subsection{Teams' solutions}

\subsubsection{Framework}
Observing that the UGC videos quality are different, besides severe compression artifacts, may also contain dark light, de-focus blur, motion blur, and noise. We propose a two - stage approach for the UGC video enhancement, and use multiple operators in each stage. The first stage for color enhancement, and the second stage for artifacts compression as well as de-noise, de-blur and texture enhancement. Our main pipeline is shown in Fig.~\ref{fig:pipline} \\We estimate the video quality and distortion type first, and process the video according to the estimated type. In the first stage, we use 3D-LUT\cite{zeng2020lut} and some maching learning methods, and the second stage are two GAN models based on Real-ESRGAN\cite{wang2021realesrgan} framework, additionally we observed that UGC videos shot with handheld devices often shake at the last frame, so we add end-frame compenstation by flow\cite{DBLP:journals/corr/RanjanB16}.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/pipeline.png}
    \caption{video enhancement pipeline.}
    \label{fig:pipline}
\end{figure}


\subsubsection{Details}
In the first stage, we used CNN as well as machine learning algorithms such as white balance and gamma correction. For the CNN model, we use Adobe 5k \cite{fivek} and self-made pictures about 10k as training data. The self - made data are generated by diffusion with prompts such as "High-contrast", "bright color" and degeneration them as LQ when trainging. \\
In the second stage, we use FFHQ\cite{karras2019stylebasedgeneratorarchitecturegenerative} and about 1000 high-quality videos from YouTube, we degenerate the high-quality videos by ffmpeg, with parameter -crf from 24 to 36, and multiple blur kernels. In addition, we use online degradation methods twice as \cite{wang2021realesrgan} when training. For the face in FFHQ, we randomly paste them in the training image pairs. The training Loss is:  $$L_{total} = L_1 + 0.1 \times L_{LPIPS} + 0.05 \times L_{GAN}$$ with a learning rate of $2 \times 10^{-4}$.


==> figures/Nobody_description/sections/teams_affiliations.tex <==
\section{Teams and Affiliations}
\textbf{NTIRE 2025 UGC Video Enhancement Teams}\\

\noindent \textit{\textbf{Team:}}\\
NoBody\\
\textit{\textbf{Members:}}\\
% Email is optional
Meisong Zheng$^1$ (zhengmeisong.zms@taobao.com), Jingyi Xu$^{1,2}$ , Chengbin Wu$^{1}$, Jiahui Liu$^{1}$, Ying Chen$^{1}$, Xin Deng$^{2}$, Mai Xu$^{2}$\\
\textit{\textbf{Affiliations:}}\\
$^1$: Department of Tao Technology, Alibaba Group, China\\
$^2$: Beihang University, Beijing, China  \\

